Groupoidal and truncated $n$-quasi-categories

We define groupoidal and $(n+k)$-truncated $n$-quasi-categories, which are the translation to the world of $n$-quasi-categories of groupoidal and truncated $(\infty, n)$-$\Theta$-spaces defined by Rezk. We show that these objects are the fibrant objects of model structures on the category of presheaves on $\Theta_n$ obtained by localisation of Ara's model structure for $n$-quasi-categories. Furthermore, we prove that the inclusion $\Delta \to \Theta_n$ induces a Quillen equivalence between the model structure for groupoidal (resp. and $n$-truncated) $n$-quasi-categories and the Kan-Quillen model structure for spaces (resp. homotopy $n$-types) on simplicial sets. To get to these results, we also construct a cylinder object for $n$-quasi-categories.

==> 2qcat.tex <==
\section{$n$-quasi-categories and Rezk $\Theta_n$-spaces}

Ara introduces in \cite{ara2014higher} $n$-quasi-categories as models for $(\infty, n)$-categories. These are presheaves on the category $\Theta_n$ which are fibrant objects for a certain model category structure on $\widehat{\Theta_n}$. Here, we consider the case $n=2$.

\begin{parag} \label{the category Delta}
We denote by $\Delta$ the category of finite ordinals $[n] = \{0 < 1 < \ldots < n\}$ and non-decreasing maps between them. There is a fully faithful inclusion $\Delta \to \Cat$, where we see each object of $\Delta$ as the category associated to the respective ordered set. 

The morphisms of $\Delta$ are generated by the face and degeneracy maps. Face maps are the maps $\delta^{i}: [n] \to [n+1]$ skipping $i$, for $0 \leq i \leq n+1$. Degeneracy maps are the maps $\sigma^i: [n+1] \to [n]$ sending both $i$ and $i+1$ to $i$, for $0 \leq i \leq n$.
\end{parag}

\begin{parag} \label{the category Theta_2}
We introduce the category $\Theta_2$ as a wreath product $\Delta \wr \Delta$, as first presented by Berger in \cite{berger2007iterated}. The objects of $\Theta_2$ are lists $[n; \mathbf{q}] = [n; q_1, \ldots, q_n]$, where $n, q_1, \ldots, q_n$ are non-negative integers. A morphism $[\alpha, \boldsymbol{\alpha}] : [m; \mathbf{p}] \to [n; \mathbf{q}]$ is the data of a morphism $\alpha: [m] \to [n]$ in $\Delta$ and of a morphism $\alpha_j: [p_i] \to [q_j]$ in $\Delta$ for every $\alpha(i-1) < j \leq \alpha(i)$, $1 \leq i \leq m$.

We shall think of $\Theta_2$ as a full subcategory of $\twocat$. An object $[n; \mathbf{q}]$ of $\Theta_2$ is represented by the 2-category freely generated by the 2-graph with $n+1$ objects $0, 1, \ldots, n$, an ordered set $\{(j,0), \ldots, (j, q_j)\}$ of  1-arrows $j-1 \to j$ for every $1 \leq j \leq n$, and one 2-arrow between any two consecutive 1-arrows between the same objects. For example, the 2-graph which generates the object $[3; 1, 0, 2]$ can be represented as below.

% https://q.uiver.app/?q=WzAsNCxbMCwwLCIwIl0sWzMsMCwiMSJdLFs2LDAsIjIiXSxbOSwwLCIzIl0sWzAsMSwiKDEsMCkiLDEseyJjdXJ2ZSI6LTN9XSxbMCwxLCIoMSwxKSIsMix7ImN1cnZlIjozfV0sWzEsMiwiKDIsMCkiLDFdLFsyLDMsIigzLDApIiwxLHsiY3VydmUiOi01fV0sWzIsMywiKDMsMikiLDEseyJjdXJ2ZSI6NX1dLFsyLDMsIigzLDEpIiwxXSxbNCw1LCIiLDEseyJzaG9ydGVuIjp7InNvdXJjZSI6MjAsInRhcmdldCI6MjB9fV0sWzcsOSwiIiwxLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfX1dLFs5LDgsIiIsMSx7InNob3J0ZW4iOnsic291cmNlIjoyMCwidGFyZ2V0IjoyMH19XV0=
\[\begin{tikzcd}
	0 &&& 1 &&& 2 &&& 3
	\arrow[""{name=0, anchor=center, inner sep=0}, "{(1,0)}"{description}, curve={height=-18pt}, from=1-1, to=1-4]
	\arrow[""{name=1, anchor=center, inner sep=0}, "{(1,1)}"', curve={height=18pt}, from=1-1, to=1-4]
	\arrow["{(2,0)}"{description}, from=1-4, to=1-7]
	\arrow[""{name=2, anchor=center, inner sep=0}, "{(3,0)}"{description}, curve={height=-30pt}, from=1-7, to=1-10]
	\arrow[""{name=3, anchor=center, inner sep=0}, "{(3,2)}"{description}, curve={height=30pt}, from=1-7, to=1-10]
	\arrow[""{name=4, anchor=center, inner sep=0}, "{(3,1)}"{description}, from=1-7, to=1-10]
	\arrow[shorten <=5pt, shorten >=5pt, Rightarrow, from=0, to=1]
	\arrow[shorten <=4pt, shorten >=4pt, Rightarrow, from=2, to=4]
	\arrow[shorten <=4pt, shorten >=4pt, Rightarrow, from=4, to=3]
\end{tikzcd}\]

\vspace{2mm}

A morphism $[\alpha, \boldsymbol{\alpha}] : [m; \mathbf{p}] \to [n; \mathbf{q}]$ corresponds to the 2-functor which sends each object $i$ of the 2-category $[m; \mathbf{p}]$ to $\alpha(i)$, each 1-morphism $(i,k)$ to the composite $$(\alpha(i), \alpha_{\alpha(i)}(k)) \circ \ldots \circ (\alpha(i-1) + 1, \alpha_{\alpha(i-1) + 1}(k))$$ when $\alpha(i) > \alpha(i-1)$ and to $\id_{\alpha(i)}$ when $\alpha(i) = \alpha(i-1)$, and each 2-morphism of $[m; \mathbf{p}]$ to the unique possible 2-morphism of $[n; \mathbf{q}]$.
\end{parag}

\begin{parag} \label{2-cellular sets}
We consider the category $\widehat{\Theta_2}$ of \textit{2-cellular sets}. The representable 2-cellular sets are denoted by $\Theta_2[n; \mathbf{q}]$. The \textit{boundary} $\partial \Theta_2[n; \mathbf{q}]$ of a representable $\Theta_2[n; \mathbf{q}]$ is the 2-cellular set generated by the non-surjective\footnote{A morphism $[\alpha; \boldsymbol{\alpha}]: [m; \mathbf{p}] \to [n; \mathbf{q}]$ is surjective if $\alpha:[m] \to [n]$ is surjective and all $\alpha_j: [p_i] \to [q_j]$ are surjective.} morphisms $[m; \mathbf{p}] \to [n; \mathbf{q}]$ in $\Theta_2$. We denote by $\delta_{n; \mathbf{q}}$ the boundary inclusion $\partial \Theta_2[n; \mathbf{q}] \to \Theta_2[n; \mathbf{q}]$.
\end{parag}

%\begin{parag} \label{spine inclusions}
%Let us define the \textit{spines} $I[n; \mathbf{q}]$. We define $I[0]$, $I[1;0]$ and $I[1;1]$ to be $\Theta_2[0]$, $\Theta_2[1;0]$ and $\Theta_2[1;1]$ respectively. For $q \geq 2$, let $$I[1; q] := \colim (\Theta_2[1;1] \leftarrow \Theta_2[1;0] \to \ldots \leftarrow \Theta_2[1;0] \to \Theta_2[1;1])$$
%where there are $q$ copies of $\Theta_2[1;1]$, the left-going arrows are given by $[\id; \delta^0]$ and the right-going arrows are given by $[\id; \delta^1]$. For $n \geq 2$, let $$I[n; \mathbf{q}] := \colim (I[1;q_1] \leftarrow \Theta_2[0] \to \ldots \leftarrow \Theta_2[0] \to I[1;q_n])$$
%where the left-going arrows are given by $[\delta^0]$ and the right-going arrows are given by $[\delta^1]$. For every $[n; \mathbf{q}] \in \Theta_2$, there is a natural inclusion $i_{n; \mathbf{q}}: I[n; \mathbf{q}] \to \Theta_2[n; \mathbf{q}]$.
%\end{parag}

\begin{parag} \label{Ara's model structure}
There is a model category structure on $\widehat{\Theta_2}$, constructed in \cite{ara2014higher} by means of Cisinki's theory of localizers, which we will call \textit{Ara's model structure for 2-quasi-categories}. The cofibrations of this model structure are monomorphisms of 2-cellular sets (and so every object is cofibrant). The fibrant objects are called \textit{2-quasi-categories}.
\end{parag}

\begin{parag}\label{left Kan extension and nerve/singular functor}
Let $F: \a \to \b$ be a functor from a small category $\a$ to a category $\b$. The \textit{evaluation (or nerve) functor} associated to $F$ is the functor $F^!: \b \to \widehat{\a}$, given by
$F^!(b)_a = \Hom_{\b}(F(a), b)$ for every $b \in \b$ and every $a \in \a$.

If $\b$ is cocomplete, the evaluation functor admits a left adjoint $F_!: \widehat{\a} \to \b$, which is the left Kan extension of $F$ along the Yoneda embedding $\a \to \widehat{\a}$.
\end{parag}

\begin{parag} \label{the strict 2-nerve}
The inclusion $\Theta_2 \to \twocat$ induces a nerve functor $N_2: \twocat \to \widehat{\Theta_2}$, which we call the \textit{(strict) 2-nerve} functor. Explicitly, for a 2-category $\cc$ and $[n; \mathbf{q}] \in \Theta_2$, we have
$$N_2 (\cc)_{n; \mathbf{q}} = \Hom_{\twocat}([n; \mathbf{q}], \cc)$$

The strict 2-nerve functor is fully faithful, cf. \cite[Theorem 1.12]{berger2002cellular}.
\end{parag}

The (strict 1-)nerve of a category is always a quasi-category. The analogous statement is not true, in general, for 2-categories.

%\begin{proposition}[Recognition principle]
%Let $X$ be...
%\end{proposition}

\begin{proposition} \label{When the strict 2-nerve of a 2-category is a 2-quasi-category}
The strict 2-nerve of a 2-category $\cc$ is a 2-quasi-category if and only if the only invertible 2-morphisms of $\cc$ are the identities.
\end{proposition}

\begin{proof}
It follows from \cite[Proposition 7.10]{ara2014higher} in the case $n=2$.
\end{proof}


